SLAKE: A Semantically-Labeled Knowledge-Enhanced Dataset for Medical Visual Question Answering

Medical visual question answering (Med-VQA) has tremendous potential in healthcare. However, the development of this technology is hindered by the lacking of publicly-available and high-quality labeled datasets for training and evaluation. In this paper, we present a large bilingual dataset, SLAKE, with comprehensive semantic labels annotated by experienced physicians and a new structural medical knowledge base for Med-VQA. Besides, SLAKE includes richer modalities and covers more human body parts than the currently available dataset. We show that SLAKE can be used to facilitate the development and evaluation of Med-VQA systems. The dataset can be downloaded from http://www.med-vqa.com/slake.

==> ISBI 2021 SLAKE/0.abstract.tex <==
% The abstract should appear at the top of the left-hand column of text, about
% 0.5 inch (12 mm) below the title area and no more than 3.125 inches (80 mm) in
% length.  Leave a 0.5 inch (12 mm) space between the end of the abstract and the
% beginning of the main text.  The abstract should contain about 100 to 150
% words, and should be identical to the abstract text submitted electronically
% along with the paper cover sheet.  All manuscripts must be in English, printed
% in black ink.
% Applying Artificial Intelligence (AI) techniques into medical domain to benefit the general public has attracted a surge of interest.
% Medical visual question answering (Med-VQA) is an emerging research field where high-level domain-specific multimodal reasoning abilities are required. Med-VQA aims to correctly answer a variety of clinical questions about various kinds of radiology images. To address the Med-VQA problem, models are supposed to learn to not only understand the visual and textual information but also acquire the underlying medical reasoning logics. However, lacking available datasets makes the research of Med-VQA progressing slowly. In this paper, we propose a novel Med-VQA dataset with sophisticated designed medical entity annotations and knowledge graph based external information. Our dataset contains XXXX. we evaluate our dataset by apply it to state-of-the-art Med-VQA methods (XXX). We observe...

%Medical visual question answering (Med-VQA) has attracted a surge of interest due to its tremendous potential in healthcare. Med-VQA aims to build machine learning algorithms that can predict the correct answer of a clinical question by automatically perceiving the information within a provided radiology image, without any help from medical experts. The wide application of Med-VQA technology will provide new diagnosis alternatives to both patients and doctors. However, the research progress of Med-VQA is hindered due to the scarcity of available dataset. In this paper, we thus present a novel bilingual Med-VQA dataset, SLAKE, which consists of comprehensive visual labels annotated by experienced physicians and an extendable external knowledge referencing mechanism. Compared with the previous Med-VQA dataset, SLAKE includes richer modalities and human body parts with bigger numbers of images and questions. We conduct comprehensive experiments via representative methods in Med-VQA to validate the feasibility and effectiveness of SLAKE and prove that SLAKE can help to develop more powerful models for Med-VQA. 

 Medical visual question answering (Med-VQA) has tremendous potential in healthcare. However, the development of this technology is hindered by the lacking of publicly-available and high-quality labeled datasets for training and evaluation. In this paper, we present a large bilingual dataset, SLAKE, with comprehensive semantic labels annotated by experienced physicians and a new structural medical knowledge base for Med-VQA. Besides, SLAKE includes richer modalities and covers more human body parts than the currently available dataset. We show that SLAKE can be used to facilitate the development and evaluation of Med-VQA systems. The dataset can be downloaded from \url{http://www.med-vqa.com/slake}.

==> ISBI 2021 SLAKE/1.introduction.tex <==
\textbf{}% (AI complete) problem to derive vqa 
% what ismed vqa and its importance
% dataset evolving status and drawbacks
% our dataset and properties
% our dataset is seminal and its excellence

Developing machines that can understand visual content and answer questions like humans is a long-standing goal of AI research. In recent years, visual question answering (VQA) has become an active field of research. Medical visual question answering (Med-VQA) is a domain-specific branch of VQA, where a clinical question comes with a radiology image and the goal is to design a system that can correctly answer the question based on the visual information of the image.

%Developing AI systems that can consciously understand and answer questions about visual information is a long-standing goal of AI research. In recent years, visual question answering (VQA) has been introduced to facilitate the research of this problem. Medical visual question answering (Med-VQA) belongs to a domain-specific branch of VQA, where a clinical question comes with a related radiology image and our purpose is to output the correct answer of this question in natural language based on the visual information of the image.
% (as a form of Visual Turing Test to benchmark performance in computer vision)
% The task simultaneously requires multiple abilities for understanding natural language, visual reasoning and fusing multi-modal features. 
% Compared with general VQA, Med-VQA has a more clear application purpose, helping patients with self-diagnosis, providing clinical decision-making for doctors, especially for inexperienced interns, and teaching everyone who is not familiar with radiology images to master basic knowledge.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.93\linewidth]{sample.pdf}
\caption{Exemplar image and questions of our SLAKE dataset.}

\label{fig:dataset}
\end{figure}


Med-VQA has a wide range of application prospects in healthcare sectors and a broad impact on the wellness of the general public. With a reliable Med-VQA system, patients can easily acquire information about their health and be more engaged in the process of decision making. For doctors, Med-VQA systems can be used to assist diagnosis by providing them a second medical opinion. The systems can also be used in clinical education to train medical professionals. Besides, Med-VQA technology can be potentially integrated into many conversational AI platforms to bring enormous benefits to healthcare industry. 

%Med-VQA has a broad impact on the wellness of the general public. Patients can use Med-VQA systems to acquire preliminary knowledge about their health. Senior doctors can reference the results of Med-VQA systems to assist their diagnosis, and these systems can also be used to the training of junior doctors. Therefore, Med-VQA can help to significantly empower our medical systems. However, the research of Med-VQA is still at its infant stage due to the lack of available datasets. 

% Recently, several datasets for Med-VQA have been proposed and significantly facilitate the development of Med-VQA. 
% Recently, although more and more researchers make contributions to general VQA, which make it popular across the board, due to high barriers of Med-VQA task itself, 
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table*}[ht]
    \centering
    %\small
    \caption{Comparison of SLAKE with VQA-RAD.}
    \label{tab:character}
    \begin{tabular}{cccccc}
    \hline
    \hline
    Dataset & \# Images & \# QA Pairs & Question Type & Language & Knowledge Graph \\
    \hline
    VQA-RAD~\cite{lau2018dataset} & 315 & 3.5K & Vision-only & EN & \XSolidBrush \\
    \hline
    \textbf{SLAKE (Ours)} & 642 & 14K & Knowledge-based \& Vision-only & \tabincell{c}{Bilingual (EN \& ZH) }  &  \Checkmark \\
    \hline
    \end{tabular}
    % \end{threeparttable}
\end{table*}

However, the research of Med-VQA is at an early stage. Unlike VQA in the general domain, where large-scale high-quality datasets~\cite{johnson2017clevr,antol2015vqa} are available, there is a lack of publicly-available and well-annotated datasets for training and evaluating Med-VQA systems. To correctly answer a clinical question about a radiology image, it requires clinical expertise and domain-specific medical knowledge, which makes it difficult to construct a realistic and accurate dataset for Med-VQA. VQA-RAD~\cite{lau2018dataset} is a first step in this direction. To our knowledge, it is the only available dataset with manual annotation, based on which several Med-VQA models have been proposed~\cite{nguyen2019overcoming,ZL-MM-20}. VQA-RAD is a diverse dataset containing a variety of different types of clinical questions, with each question type sufficiently represented. But it does not provide semantic labels, e.g., labeled segmentations of organs and tumors or bounding boxes on objects, which are essential for training a Med-VQA model to find the region of interest in an image to answer complex clinical questions. Moreover, a practical Med-VQA system needs to exploit external knowledge apart from visual content to answer complex compositional questions involving inquires such as ``the functionality of an organ'', ``the cause of a disease'', or ``the treatment of a disease'', which is also not supported in VQA-RAD. 


%  ``the treatment of a disease''
% In addition, the questions in VQA-RAD~\cite{lau2018dataset} only focus on the visual contents, meaning that the models could answer by directly analysing the question and image alone. However, for a health-care and educating system, this kind of question is not enough. The question, which contains external knowledge such as ``the function of some organs'', ``the cause of a disease'', or ``the treatment of a disease'', could not be solved by systems trained on the VQA-RAD~\cite{lau2018dataset}.

 %Remarkably, solving clinical questions requires a large range of medical expert knowledge and complex medical domain-specific diagnosis skills, leading to the difficulty of designing realistic datasets for Med-VQA. As far as we know, there is only one manually annotated dataset available - VQA-RAD~\cite{lau2018dataset} on which several methods have been proposed~\cite{nguyen2019overcoming,10.1145/3394171.3413761}. Like datasets~\cite{johnson2017clevr,antol2015vqa} in general VQA domain, VQA-RAD contains a variety of clinical questions to guarantee its diversity while keeping the numbers of different types of questions balanced in general. However, to tackle the inherent complexity of Med-VQA, annotating the question and image pair at a high level without sophisticated visual entity labels and external knowledge is not enough and hinders developing more powerful Med-VQA systems.
% to guarantee its reliability
% For the VQA-RAD dataset~\cite{lau2018dataset}, despite its construction is completed by professional radiotherapy technicians and related medical workers, there are still some flaws in it, e.g., the images in it without visual annotations. This design of dataset will make Med-VQA more challenging. On one hand, it is difficult for non-medical researchers to understand the medical visual concepts without any visual tips. It creates a high barrier that reduces the focus in this VQA domain. For example, the question, ``is there an appendix in the picture?'', will naturally lead to think whether the appendix exists in this image and where it locates. On the other hand, models used for visual reasoning could not deeply understand images. They could only learn part of each image under the guidance of the concomitant questions. When models meet the new questions about images in the test stage, wrong answers will occur in a high probability.

To fill these gaps, we construct a \textbf{s}emantically-\textbf{la}beled \textbf{k}nowledge-\textbf{e}nhanced (SLAKE) dataset with accurate visual and textual annotations and an extendable knowledge base for Med-VQA. It takes our team more than half of a year to complete all the tasks, including building the annotation system, constructing the medical knowledge graph (KG), selecting and labeling images, generating questions, and analyzing the dataset.
% In addition, our dataset contains bilingual questions, i.e., English and Chinese.
% To ensure that the questions and images are more in line with clinical and patient applications, SLAKE is manually constructed by professional physician.
As shown in Figure~\ref{fig:dataset}, for each radiology image, we provide two kinds of visual annotations: \emph{masks} for semantic segmentation and \emph{bounding boxes} for object detection. Besides basic clinical questions, we also design compositional questions that require multiple reasoning steps, and knowledge-based questions like~\cite{wang2018fvqa} that involve external medical knowledge. In general, questions in SLAKE can be categorized as vision-only questions and knowledge-based questions. We provide detailed annotations to distinguish the two types of questions and guide the Med-VQA model to search for answers on the knowledge graph. Besides these new features, SLAKE is designed to be an English-Chinese bilingual dataset to broaden its application range. Further, SLAKE covers more body parts (e.g., neck and pelvic cavity) and more types of questions (e.g., shape and KG-related) than VQA-RAD. A comparison between our SLAKE and VQA-RAD is provided in Table~\ref{tab:character}. 

%% time line

% Our team continuously spend nearly half a year to complete our SLAKE dataset, including annotation system production, knowledge graph establishment, image labeling, question generation, dataset evaluation.
% Because there are two kinds of questions in our dataset, we provide detailed labels in form of triplet for each of them to judge category and predict the parts of the knowledge-based questions that involve external knowledge. 
%Besides these designing mechanism innovations, SLAKE is also enhanced to contain more basic information. To broaden the application of our dataset, we include bilingual questions and knowledge graphs (i.e., English and Chinese) in SLAKE. Moreover, compared with previous Med-VQA datasets, SLAKE contains images with more body parts (e.g., neck and pelvic cavity) and more elements (e.g., color and shape) in questions.

% Considering that the modality of medical images are different when checking different parts of the body. For the images of our SLAKE dataset, we mainly have three kinds: CT, MRI and X-Ray.

% For the composition of our SLAKE dataset, compared with VQA-RAD~\cite{lau2018dataset} with three parts of the body, head, chest, and abdomen, we extend the coverage with two additions, neck and pelvic cavity. Considering that the modality of medical images are different when checking different parts of the body, we mainly collect three types: CT, MRI and X-Ray. Meanwhile, we also increase the number of images. Specifically, there are 140 head CTs or MRIs, 41 neck CTs, 219 chest X-Rays or CTs, 201 abdomen CTs or MRIs, and 41 pelvic cavity CTs. Definitely, the number of questions also grows along with increasing images.  Moreover, we empower the complexity of questions manifested as the introduction of content types such as  ``Color'', ``Shape'', ``Quality'', etc.

% Definitely, the number of questions also grows along with increasing images. 
% we extend the coverage and number of medical images. It covers most parts of the body except for limbs and blood vessels, mainly the head, neck, chest, abdomen, and pelvic cavity. Specifically, there are 140 head single-slice CTs or MRIs, 
% Definitely, the number of questions also grows along with increasing images.



In summary, our contributions are two-fold:
\begin{itemize}
	\item We create SLAKE, a large-scale, semantically annotated, and knowledge-enhanced bilingual dataset for training and testing Med-VQA systems. 
% 	With these abundant information, we expect our dataset can help to build a fertile ground for the development of Med-VQA.
	\item We experiment with representative Med-VQA methods to show that SLAKE can be used as a benchmark to train systems to solve practical and complex tasks. 
\end{itemize} 

% \vspace{-1em}
% In summary, we make three main contributions: (1) the rich visual annotations for each image helping both researchers and models understand medical image reasoning; (2) diverse question types, vision-only, knowledge-based, and bilingual, could make the Med-VQA system meet more requirements and more widely used; (3) wider range of medical images and larger dataset. As a new dataset in Med-VQA, SLAKE fill many blanks for the current domain and provide a solid foundation for development. We hope it can serve as a bridge to a truly widely used medical system in the future. 

% (1) \textbf{rich visual annotations}: for each image in (2) \textbf{diverse question types.} (3) \textbf{extensive medical images.}



==> ISBI 2021 SLAKE/2.dataset.tex <==
% The SLAKE dataset mainly focuses on cross-modal reasoning on the radiology images and medical knowledge graph under the guidance of bilingual question features. 
In this section, we elaborate on the construction of our SLAKE dataset. In general, we ensure the diversity of the dataset in terms of modalities (e.g., CT, MRI, and X-Ray), covered body parts (e.g., head, neck, and chest), and question types (e.g., vision-only, knowledge-based, and bilingual). 


% \begin{table}[t]
%     \centering
%     \small
%      \caption{Image composition of our SLAKE dataset.}
%       \begin{tabular}{ccccc}
%  \hline
% \hline
%   Body Part& Number&Modality &Disease\\
%   \hline
%     Head           &  141  &    CT, MRI   &   \tabincell{c}{Brain Edema\\Brain Tumor}	\\
%  \hline
%     Neck           &  41   &	CT        &   Esophagus Cancer 	\\
%     \hline
%     \multirow{7}{*}{Chest}  &  \multirow{7}{*}{219}  &	CT &  Lung Cancer\\
%     \cline{3-4}
%                             &                        &  X-Ray   & \tabincell{c}{
% Atelectasis\\Cardiomegaly\\Effusion\\Infiltration\\Mass\\Pneumothorax}


% \\
% \hline
%     Abdomen        &  201  &	CT, MRI   &   \tabincell{c}{Liver Cancer\\
% Kidney Cancer}  	
%     \\
%     \hline
%     Pelvic Cavity  &  41   &    CT        &   - 	\\

%     \hline
%     \hline
%     \end{tabular}
%     \label{tab:image_statistic}
% \end{table}

% The main characteristics and difference of VQA-RAD~\cite{lau2018dataset} and our SLAKE are shown in Table~\ref{tab:character}.  
% Firstly, we select radiology images from open resources and annotate each of them with two kinds of labels. Secondly, based on the visual concepts of selected images, we manually construct the corresponding knowledge graph. Then, pre-define content types of questions and generate QA pairs from the visual concepts and knowledge graph. Finally, balance the whole dataset and randomly divide it for training, validating and testing according to the rational proportion. Specifically, it consists of $642$ images, 14k questions of varied types, and a self-built medical knowledge graph with 6k selected entities.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pie.png}
    \caption{Left: proportions of images of five body parts. Right: distribution of the content types of questions.}
    \label{fig:proportion}
\end{figure}
%reviewer 3
\subsection{Image Acquisition and Annotation} 
\label{sec:selection}
We select radiology images, covering healthy and unhealthy cases, from three open source datasets \cite{simpson2019large}\footnote{\url{http://medicaldecathlon.com}} \cite{wang2017chestx}\footnote{\url{https://nihcc.app.box.com/v/ChestXray-NIHCC}} \cite{CHAOSdata2019}\footnote{\url{https://doi.org/10.5281/zenodo.3431873}}. From \cite{wang2017chestx}, we randomly select $179$ chest X-Ray images and keep the original disease labels. From \cite{simpson2019large} and \cite{CHAOSdata2019}, we randomly choose $463$ single-slice images from $3$\emph{D} volume cases. Then, experienced physicians label organs and diseases as detailed as possible with ITK-SNAP~\cite{py06nimg}\footnote{\url{http://www.itksnap.org}} as shown in Figure~\ref{fig:dataset}. 

% From \cite{wang2017chestx}, we randomly select $179$ chest X-Ray images and keep the original disease labels, such as pulmonary nodules, pneumonia, etc. From \cite{simpson2019large} and \cite{CHAOSdata2019}, we randomly select $463$ images while maintaining the integrity of the data.

% in proportion to the number of organs in five body parts. 

% We , including 140 head CTs or MRIs, 41 neck CTs, 219 chest X-Rays or CTs, 201 abdomen CTs or MRIs, and 41 pelvic cavity CTs. brain edema, brain tumor, esophagus cancer, lung cancer, atelectasis, cardiomegaly, effusion, infiltration, mass, pneumothorax, liver cancer, kidney cancer. 

In total, we annotate 642 images, including 12 diseases and 39 organs of the whole body. The diseases mainly include cancer (e.g., brain, liver, kidney, lung, etc.), and thoracic diseases (e.g., atelectasis, effusion, mass, pneumothorax, etc.). The images include 140 head CTs or MRIs, 41 neck CTs, 219 chest X-Rays or CTs, 201 abdomen CTs or MRIs, and 41 pelvic cavity CTs. The distribution is shown in Figure~\ref{fig:proportion} (Left). Among these images, there are 282 CTs, 181 MRIs, and 179 X-Rays. All CTs and MRIs are axial single-slice. The number of images for each body part is set based on the complexity of the body part. For example, the number of diseases and organs in abdomen is much more than that in neck, so there are more images of abdomen than neck in the dataset. 



\subsection{Knowledge Graph Construction}
%traverse
To answer questions that require external medical knowledge, we construct a medical knowledge graph centered on organs and related diseases, which are the main objects of radiology images. 
We extract a set of 52.6K triplets \emph{\textless head, relation, tail\textgreater} with medical knowledge from OwnThink\footnote{\url{https://www.ownthink.com}}, a large-scale knowledge base built on Wikipedia. Here, \emph{head} and \emph{tail} are entities such as organ, disease, etc., and \emph{relation} represents the relationship between entities, such as function or treatment. Then, we traverse the set to retrieve triplets related to organs and the corresponding diseases. We further clean the data by manually filtering out some entities that are not presented in medical images such as gastritis and nephritis.
% However, many of them are not useful because the entities could not be seen on radiology images, such as gastritis, nephritis. Therefore, we filter the triplets to make them more suitable for knowledge-based visual reasoning.


\begin{table}[t]
    \centering
    \small
     \caption{Statistics of questions in our SLAKE dataset.}
      \begin{tabular}{c|cccc}
  \hline
  \hline
  &\textbf{Training set}&\textbf{Validation set}&\textbf{Test set}\\
  \hline
   
     Plane       &	931  &   173  &	176	\\
     Quality    &	535  &	109  &	118	\\
     Modality    &	1072  &	203  &	217   \\
     Position	 &  1876	&   412 &	390  \\
     Organ      &	2125 &	462	&   454	\\
     KG          &	1202 &	278	&   260 \\
     Abnormal	 &  1230	&   245  &	221   \\
     Color      &	424	&   108	&   115   \\
     Shape       &	157	&   42	&   46   \\
     Size      &	297	&   77 &	73   \\
    \hline
    Total&{\bf 9849}&{\bf 2109}&{\bf 2070}\\
    \hline
    \hline
    \end{tabular}
    \label{tab:statistic}
\end{table}



Next, in order to extensively cover frequently referenced knowledge, we refine the filtered triplets with the following rules: (1) The triplets about an organ must describe its function or body system; (2) The triplets about a disease must describe the symptoms, locations, causes, treatment or prevention methodologies. Some examples are shown in Table~\ref{tab:examle_kg}.

%(1) For each organ, the triplet set must contain the organ's function and body system; (2) For the diseases, the triplet sets must contain symptoms, locations, causes, treatment and prevention methodologies, as shown in Table~\ref{tab:examle_kg}. 

Finally, we make the triplets bilingual and obtain $2603$ triplets in English and $2629$ triplets in Chinese.




\subsection{Question Generation}
\label{sec:qg}

%reviewer2 
Questions are proposed by experienced doctors. To accelerate this process, we develop an annotation system. In this system, we first pre-define a question template for each body part (i.e., head, neck, chest, abdomen, and pelvic cavity). Then, we define ten different content types (e.g., \emph{modality}, \emph{position}, \emph{color}) for the questions, as shown in Table~\ref{tab:statistic} and Figure~\ref{fig:proportion} (Right).
% more clear 
In each template, we provide many candidate questions for each content type. For example, the candidate question for a head image with the content type \emph{organ} may be ``Is this a study of the head?'' or ``What organ system is imaged?''. Physicians could choose those candidate questions or amend or even rewrite them entirely based on their personal clinical experience. The flexibility of our annotation system ensures the question diversity of SLAKE. Note that because we provide different candidates for bilingual questions, the number and content of them in our dataset are not the same. 

%Additionally, because the candidate questions are randomly selected from templates, the number of questions varies from language to language and there is no translation relationship between bilingual questions of one image.

% change <vhead>
Moreover, we provide semantic label for each question. Specifically, we use  \emph{\textless vhead, \_ , \_\textgreater} (\emph{vhead} is a placeholder) to denote vision-only questions. For a knowledge-based question like ``Which organs in this image belong to the digestive system?'', we denote it as \emph{\textless vhead, belong to, digestive system\textgreater}. Such labeling helps to distinguish question type and identify the part of the question involving external knowledge.

% 
Besides, recent studies~\cite{agrawal2016analyzing,zhang2016yin} have shown that VQA models may be susceptible to the statistical bias of answer distribution of the datasets. To mitigate the inherent bias of SLAKE, we make the answers balanced in general such that the VQA model will not be biased to the most popular answer in the dataset.
For example, for the question ``Is this a study of the abdomen?'',  we make sure this question is asked with abdomen images and non-abdomen images with $50-50$ chance, thereby keeping the numbers of ``Yes'' and ``No'' balanced.
% In total, the number of answers ``Yes'' and ``No'' for it would be balanced as long as the number of images in the abdomen and other parts is proportional. be trapped by the low hanging fruit of merely outputting

\begin{table}[t]
 
  \centering
  \small
%   \fontsize{7}{8}\selectfont
%   \begin{threeparttable}
  \caption{Examples of our medical knowledge graph.}
  \label{tab:examle_kg}
   \centering
  \small
%   \renewcommand\arraystretch{1.2}
  \begin{tabular}{c|c}
  \hline
    \hline
     & Examples \\  \hline
    \multirow{3}{*}{Organ} &  {\emph{\textless Heart, Function, Promote blood flow\textgreater}}\\ 
     &  {\emph{\textless Kidney, Belong to, Urinary System\textgreater}}\\
     &  {\emph{\textless Duodenum, Length, 20-25cm\textgreater}}\\
    \hline
    \multirow{5}{*}{Disease} &  {\emph{\textless Pneumonia, Location, Lung\textgreater}}\\ 
     &  {\emph{\textless Lung Cancer, Cause, Smoke\textgreater}}\\ 
     &  {\emph{\textless Brain Tumor, Symptom, Visual impairment\textgreater}}\\ 
     &  {\emph{\textless Cardiomegaly, Treatment, Medication\textgreater}}\\ 
     &  {\emph{\textless Atelectasis, Prevention, Exercise\textgreater}}\\ 
    \hline
    \hline
    \end{tabular}
    % \end{threeparttable}
\end{table}

\subsection{Dataset Splitting}
Here, we describe how to divide the obtained 642 images with 14,028 question-answer pairs and 5232 medical knowledge triplets for the training and evaluation of Med-VQA models. 

In general, the splitting aims to provide a reliable measure of the generalization ability of the model trained on our dataset.
Specifically, we split the dataset into training ($70\%$), validation ($15\%$), and test ($15\%$) sets at the image level. The images in our dataset are split with the 75:15:15 ratio in each of the $8$ categories: ``head CT'', ``head MRI'', ``neck CT'', and ``chest X-Ray'', ``chest CT'', ``abdomen CT'', ``abdomen MRI'', and ``pelvic cavity CT''. Note that we only divide the images but the questions associated with each image are not split. 

%reviewer 3, split

% To reasonably examine the performance of a model on SLAKE, we split the dataset into training ($70\%$), validation ($15\%$), and test ($15\%$) sets at the image level. 
% In general, we split the dataset into training ($70\%$), validation ($15\%$), and test ($15\%$) sets at the image level. 
% % change
% Since the images are about different body parts and in different modalities, randomly splitting them may result that there are some images in the test set whose features are never seen in the training set~\cite{teney2016zero}. It would then be difficult, if not possible, for the model to correctly answer the accompanied questions during testing. Thus, we split the images within each of the $8$ categories ``head CT'', ``head MRI'', ``neck CT'', ``chest X-Ray'', ``chest CT'', ``abdomen CT'', ``abdomen MRI'', and ``pelvic cavity CT'', with the 75:15:15 ratio. 
% To ensure the test set can be representative enough for measuring the generalization , 

% In our dataset, we have $7$ kinds of units and independently sample images from them according to the above proportion. 
Besides, since VQA is usually formulated as a classification task~\cite{nguyen2019overcoming,ZL-MM-20,yang2016stacked},
%usually formalized as classification problem we fooloew the convention
we follow the convention and make sure answers in the test set must appear in the training set. Finally, the images are split into $450$ for training, $96$ for validating, and $96$ for testing. The number of questions of different type in each set is shown in Table~\ref{tab:statistic}. 

% To avoid inherent bias in the dataset, we keep the number of specific counterpart answers (like ``YES'' or ``NO'') balanced in general such that statistical models will not be trapped by the low hanging fruit of merely outputting the answer that occupies the larger proportion in the dataset


==> ISBI 2021 SLAKE/3.base.tex <==
% \begin{Fig.}[t]
%     \centering
%     \includegraphics[width=0.92\linewidth]{structure.png}
% \caption{The structure of system designed for SLAKE.}
% \label{fig:structure}
% \end{Fig.}

% where to clarify the meaning of the open-ended and closed-ended

% intro baseline -> huge gap for using -> questions balanced -> annotations useful
\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{structure.png}
    \caption{The Med-VQA framework on our SLAKE dataset.}
    \label{fig:structure}
\end{figure}




% In this section, we conduct assorted experiments to comprehensively evaluate our SLAKE dataset proposed in Section~\ref{sec:dataset}. In order to correctly handle different types of tasks in SLAKE, we design a structure that simultaneously processes vision-only and knowledge-based bilingual questions. Then we apply current state-of-the-art methods to obtain reliable results as strong baselines, revealing the challenge of dataset. Meanwhile, it can be seen by analyzing the accuracy of questions with different answer types that the number of questions is balanced. Finally, we do the experiments to verify that the semantic annotations for both vision and text we provide are effective. 
In this section, we conduct extensive experiments to comprehensively evaluate our SLAKE dataset. To be elaborated later, Table~\ref{tab:exp} demonstrates the usefulness and the challenge of SLAKE with commonly used Med-VQA methods. To show the effectiveness of the constructed medical knowledge graph, we conduct an ablation study presented in Table~\ref{tab:KG_exp}.
\subsection{Experiment Setup}
\label{sec:setup}
The pipeline of our experiments is illustrated in Figure~\ref{fig:structure}. We experiment with a commonly used Med-VQA framework, stacked attention network (SAN)~\cite{yang2016stacked}, on SLAKE.
% Considering modules selection in whole structure, 
% In general, the architecture of our experiments is shown in Figure~\ref{sec:baseline}
We use VGG16~\cite{simonyan2014very} to extract visual features from radiology images. For bilingual questions, we first design a bilingual tokenizer to create bilingual word embeddings for the English questions and Chinese questions respectively. 
Then, a 1024\emph{D} - LSTM is applied to extract textual semantics from these embeddings and classify types of questions. There are two sub pipelines in Figure~\ref{fig:structure}. Given the extracted visual and textual features, vision-only tasks will be directed to the multimodal fusion module of SAN to create fused features for classification. For knowledge-based tasks, question-related embeddings extracted from the knowledge graph will be combined with the multimodal fused features for classification. 
% The experiments are executed on an Ubuntu server with Titan XP GPUs. 
% When meet the knowledge-based ones, we would combine additional question related embedding extracted from knowledge graph. 

% Finally, the MLPs could be adopted as classifier to reason final answers.In this paper, the metric we used for evaluating dataset is accuracy.

\subsection{Dataset Analysis}
We report the results for vision-only and knowledge-based questions in Table~\ref{tab:exp} and Table~\ref{tab:KG_exp} respectively. Answers of ``closed-ended'' questions are limited multiple-choice options,  while answers of ``open-ended'' questions are free-form texts. Open-ended questions are generally harder to answer than closed-ended ones. 
%Open-ended questions are generally harder to answer than closed-ended ones. 
\begin{table}[t]
    \centering
    \caption{Accuracy for vision-only questions (\%).}
    \label{tab:exp}
    \begin{tabular}{cc|ccc}
    \hline
    \hline
    \multirow{2}{*}{Language} & \multirow{2}{*}{Models}  & \multirow{2}{*}{Overall} &  \multirow{1}{*}{Open-}  & \multirow{1}{*}{Closed-} \\
          &     &    &   ended &  ended   \\
    \hline
    % &ResNet+SAN &  73.85    &     73.48      &     74.39    \\
    % ResNet+BAN &  74.97    &     74.24      &     \textbf{76.01}         \\
    \multirow{2}{*}{English} & VGG+SAN&   72.73    &     70.34      &     76.13\\
        &   VGG\emph{seg}+SAN &   \textbf{75.36}    & \textbf{72.20}&    \textbf{79.84} \\
    \hline
    Chinese & VGG+SAN& 74.27 & 73.64& 75.20 \\
    \hline
    % \multirow{2}{*}{Knowledge-Based}&\multirow{2}{*}{English} & VGG+SAN & 70.65 & 73.65& 63.95\\
    % & & VGG+SAN+KG & 73.09 & 71.65 & 76.32\\
    \hline
    \end{tabular}
\end{table}
\begin{table}[t]
    \centering
    \caption{Accuracy for knowledge-based questions (\%).}
    \label{tab:KG_exp}
    \begin{tabular}{cc|c}
    \hline
    \hline
     Language & Models    &   Overall   \\
    \hline
    \multirow{2}{*}{English}& VGG+SAN & 70.27 \\ %& 73.65& 63.95\\
        &VGG+SAN+KG & \textbf{72.30} \\% & 71.65 & 76.32\\
    \hline
    Chinese & VGG+SAN+KG & 75.01 \\ %& 73.65& 63.95\\{74.91} \\% & 71.65 & 76.32\\
    \hline
    \hline
    \end{tabular}
\end{table}
%huge gap jieshi

\textbf{Vision-only questions.} In Table~\ref{tab:exp}, we report the results in accuracy for vision-only questions in both English and Chinese. Compared with VQA in the general domain, clinical questions in Med-VQA need to be answered as accurate as possible because they relate to health and safety. It can be seen that the baseline models achieve accuracy of around $73\%$ which is still far away from practical use in the medical domain. There is a wide gap between this and clinical standard, which shows that SLAKE is challenging. Moreover, it can be seen that the overall accuracy is roughly the average of those of open-ended and closed-ended questions, proving that the question distribution of SLAKE is balanced.
        
Besides, to demonstrate the usefulness of the semantic visual annotations elaborated in Section~\ref{sec:selection}, we design another model, VGG\emph{seg}+SAN. First, we pretrain a fully convolutional network (FCN) with VGG backbone by the segmentation task of radiology images with respect to the \emph{mask} labels in the training set.
Then, we initialize the VGG backbone in the Med-VQA model with the pretrained parameters. The overall accuracy increases from $72.73\%$ to $75.36\%$ with a $2.6\%$ improvement, which shows that our semantic visual annotations could improve the reasoning abilities of the model.

\textbf{Knowledge-based questions.} We leverage the self-built medical knowledge graph to answer knowledge-based questions. First, we randomly initialize an embedding for each entity in the knowledge graph and use the TransE~\cite{bordes2013translating} method to enforce the embeddings of the entities in each triplet, \emph{\textless head, relation, tail\textgreater}, to satisfy: $ \emph{head} \boldsymbol{+} \emph{relation} \boldsymbol{\approx} \emph{tail}$. Then, based on the semantic textual annotations (Section~\ref{sec:qg}), we train two LSTMs to predict the words for the ``relation'' and ``tail'' of a question separately. Next, we find the corresponding entity embeddings of the relation and tail from the graph and use them to obtain the head entity embedding based on the above approximate equation, which is then combined with the fused multimodal features for final prediction. The result is reported in Table~\ref{tab:KG_exp}.
For comparison, we also try to predict answers without using the knowledge graph. The result is $2.0\%$ lower, indicating that the constructed knowledge graph is informative and it is helpful to leverage external structural knowledge to tackle knowledge-based questions.

% which learns a embedding for knowledge graph.
% For each triplets \emph{\textless head, relation, tail\textgreater} in the knowledge graph, transE learns the embedding $h$, $r$ and $t$ for head, relation and tail respectively, which maintain $h + r = t$. % implementation of thunlp
% We use Stacked Attention Network(SAN) \cite{kim2018bilinear} to extract multimodal features of images and questions. Here we use VGG16 to extract image feature and LSTM for question feature.
% In the meanwhile, we train 2 LSTMs to classify the relation and the tail in questions separately so that we can combine the embedding of knowledge graph with the multimodal feature.

% The procedure is shown in bottom-right part of Fig.  \ref{fig:structure}. The multimodal feature and the embedding are fed into a MLP and the model can give the answer to a question. For comparison, we use a single SAN as baseline. we run two model 5 times seperately and report the average accuracy.
% The result is shown in Table \ref{tab:KVQA_res}. 



==> ISBI 2021 SLAKE/4.conclusion.tex <==
% In this paper, we introduced XMVQA for bilingual reasoning on radiology images and knowledge graph. We described its construction process and composition in detail. For each task in dataset, we did experiments and provided strong baselines. As a new dataset in Med-VQA, it filled many gaps for this domain. We strongly hope that XMVQA could promote the development of medical visual question answering.

We have introduced SLAKE, a new large bilingual dataset to facilitate the training and evaluation of Med-VQA systems.
% and to advance the research of Med-VQA fundamentally. 
SLAKE is a diverse and balanced dataset containing rich visual and textual annotations and a unique medical knowledge graph, which allows the development of more powerful Med-VQA systems. Remarkably, our experiments show that the semantic annotations and external knowledge can significantly improve the performance of standard Med-VQA models. We hope SLAKE will serve as a stepping stone to push forward the research of Med-VQA.
% To avoid inherent bias in the dataset, we keep the number of specific counterpart answers (like ``YES'' or ``NO'') balanced in general such that statistical models will not be trapped by the low hanging fruit of merely outputting the answer that occupies the larger proportion in the dataset.
% We have struck the diversity of SLAKE in terms of modalities (e.g., CT, MRI and X-Ray), and body parts (e.g., head, neck and chest), and question types (e.g., vision only, knowledge-based, and bilingual).  and our dataset will be released after the acceptance


==> ISBI 2021 SLAKE/5.ethical.tex <==
This research study was conducted retrospectively using human subject data made available in open access by~\cite{simpson2019large,CHAOSdata2019,wang2017chestx}. Ethical approval was not required as confirmed by the license attached with the open access data.


==> ISBI 2021 SLAKE/6.acknowledgement.tex <==
We would like to thank the anonymous reviewers for their helpful comments. Thanks to Lau et al~\cite{lau2018dataset} for their pioneering work in Med-VQA, NIH Clinical Center for sharing their open access dataset~\cite{wang2017chestx}, and all the doctors and medical students who helped with this research. This research was supported by the grant of P0030935 (ZVPY) funded by PolyU (UGC).
